Specification-Guided Learning of Nash Equilibria with High Social Welfare

Reinforcement learning has been shown to be an effective strategy for automatically training policies for challenging control problems. Focusing on non-cooperative multi-agent systems, we propose a novel reinforcement learning framework for training joint policies that form a Nash equilibrium. In our approach, rather than providing low-level reward functions, the user provides high-level specifications that encode the objective of each agent. Then, guided by the structure of the specifications, our algorithm searches over policies to identify one that provably forms an $\epsilon$-Nash equilibrium (with high probability). Importantly, it prioritizes policies in a way that maximizes social welfare across all agents. Our empirical evaluation demonstrates that our algorithm computes equilibrium policies with high social welfare, whereas state-of-the-art baselines either fail to compute Nash equilibria or compute ones with comparatively lower social welfare.

==> Figure/gridworldfigure.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/gridworld_spec0.pdf}
\caption{Spec 0}
\label{Fig:GridWorld44spec0}
\end{subfigure}
\quad
%\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/gridworld_spec1.pdf}
\caption{Spec 1}
\label{Fig:GridWorld44spec1}
\end{subfigure}
\quad
%\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/gridworld_spec2.pdf}
\caption{Spec 2}
\label{Fig:GridWorld44spec2}
\end{subfigure}
%\hfill         
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/gridworld_spec3.pdf}
\caption{Spec 3}
\label{Fig:GridWorld44spec3}
\end{subfigure}
\quad
%\hfill          
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/gridworld_spec4.pdf}
\caption{Spec 4}
\label{Fig:GridWorld44spec4}
\end{subfigure}
\quad
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{Plot/gridworld_spec5.pdf}
\caption{Spec 5}
\label{Fig:GridWorld44spec5}
\end{subfigure}
\quad
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{Plot/gridworld_spec6.pdf}
\caption{Spec 6}
\label{Fig:GridWorld44spec6}
\end{subfigure}
\caption{Learning curves for the Gridworld environment. 
Results are averaged over 10 runs. $x$-axis denotes the number of samples. $y$-axis denotes the average of probability of success for all agents.}
\label{Fig:GridWorld44}
\end{figure*}


==> Figure/sortworlddeterministc.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/sortworld_spec0.pdf}
\caption{Spec 0}
\label{fig:16rooms9}
\end{subfigure}
\quad
%\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/sortworld_spec1.pdf}
\caption{Spec 1}
\label{fig:16rooms10}
\end{subfigure}
\quad
%\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/sortworld_spec2.pdf}
\caption{Spec 2}
\label{fig:16rooms11}
\end{subfigure}
%\hfill         
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/sortworld_spec3.pdf}
\caption{Spec 3}
\label{fig:16rooms12}
\end{subfigure}
\quad
%\hfill          
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Plot/sortworld_spec4.pdf}
\caption{Spec 4}
\label{fig:16rooms13}
\end{subfigure}
\quad
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{Plot/sortworld_spec5.pdf}
\caption{Spec 5}
\label{fig:scalability}
\end{subfigure}
\quad
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{Plot/sortworld_spec6.pdf}
\caption{Spec 6}
\label{fig:scalability}
\end{subfigure}
\quad
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{Plot/sortworld_spec7.pdf}
\caption{Spec 7}
\label{fig:scalability}
\end{subfigure}
\caption{Learning curves for SortWorld (Deterministic) environment. 
Results are averaged over 10 runs. $x$-axis denotes the number of samples. $y$-axis denotes the average of probability of success for all agents.}
\label{Fig:16Rooms}
\end{figure*}

